Random Function Descent

Classical worst-case optimization theory neither explains the success of optimization in machine learning, nor does it help with step size selection. In this paper we demonstrate the viability and advantages of replacing the classical 'convex function' framework with a 'random function' framework. With complexity $\mathcal{O}(n^3d^3)$, where $n$ is the number of steps and $d$ the number of dimensions, Bayesian optimization with gradients has not been viable in large dimension so far. By bridging the gap between Bayesian optimization (i.e. random function optimization theory) and classical optimization we establish viability. Specifically, we use a 'stochastic Taylor approximation' to rediscover gradient descent, which is scalable in high dimension due to $\mathcal{O}(nd)$ complexity. This rediscovery yields a specific step size schedule we call Random Function Descent (RFD). The advantage of this random function framework is that RFD is scale invariant and that it provides a theoretical foundation for common step size heuristics such as gradient clipping and gradual learning rate warmup.

==> sections/extensions/acceleration.tex <==
\section{Momentum}
While the first step of RFD is optimal as it minimizes the conditional
expectation, it is not necessarily optimal for multiple steps. In
ill-conditioned problems, where the cost function forms a narrow ravine,
gradient methods are known to converge slowly. As can be seen in
Figure~\ref{fig: condition and rfm} RFD exhibits the symptoms of an
ill-conditioned problem. Grafting RFD step sizes onto deterministic momentum, we
achieve competitive results without the need for hyperparameter tuning
(Figure~\ref{fig: condition and rfm}).

\begin{figure}
	\centering
	\def\svgwidth{0.24\textwidth}
	\input{graphics/grad_projections_1000dim_30steps_s=0.05_RFD.pdf_tex}
	\hspace*{-0.2cm}
	\def\svgwidth{0.25\linewidth}
	\input{graphics/1000dim_30steps_s=1.0_Adam_NAdam_RFM_RFD.pdf_tex}
	\hspace*{-0.2cm}
	\def\svgwidth{0.25\linewidth}
	\input{graphics/1000dim_30steps_s=0.1_Adam_NAdam_RFM_RFD.pdf_tex}
	\hspace*{-0.2cm}
	\def\svgwidth{0.25\linewidth}
	\input{graphics/1000dim_30steps_s=0.05_Adam_NAdam_RFM_RFD.pdf_tex}
	\caption{
		30 steps of \ref{rfd} on a 1000-dimensional Gaussian random function
		with squared exponential covariance \eqref{eq: sqExp covariance model}.
		Left: Projecting these gradients onto each other measures the
		similarity of their direction. This ``similarity score'' is plotted as a heat-map
		(\(\scale=0.05\)). The checkerboard pattern suggests gradients zig-zag
		on this random function (a characteristic of narrow ravines -- high condition
		numbers). While this is only a single realization, the pattern is always
		visible no matter the random seed.
		The remaining figures plot \((n, \Cost(\param_n))\) for
		\(\param_n\) generated by different algorithms. Length scales of
		\eqref{eq: sqExp covariance model} left to right: \(\scale=1\),
		\(\scale=0.1\) and \(\scale=0.05\). As Adam
		\citep{kingmaAdamMethodStochastic2015} and NAdam
		\citep{dozatIncorporatingNesterovMomentum2016} are not scale
		invariant, this is equivalent to tuning their step size.
		\ref{rfd} and \rfm{} remain invariant.
	}
	\label{fig: condition and rfm}
\end{figure}

While classic (heavy-ball) momentum
\citep{polyakMethodsSpeedingConvergence1964} (HBM)
% \[
% 	\tag{HBM}
% 	\param_{n+1}
% 	= \param_n + \beta (\param_n - \param_{n-1}) - \stepsize \nabla\Cost(\param_n)
% \]
attains optimal convergence speed on quadratic functions,\footnote{
	In the set of algorithms which select \(\param_{n+1}\) from the linear hull
	of gradients \(\nabla\Cost(\param_0),\dots\nabla\Cost(\param_{n})\)
	\citep[Sec~2.1.4]{gohWhyMomentumReally2017,nesterovLecturesConvexOptimization2018}.
}
it can fail to converge on more general functions
\citep[Sec~4.6]{lessardAnalysisDesignOptimization2016}. So we choose
Nesterov's momentum, which breaks apart the two updates to the parameters
\(\param_n\) of HBM. It first applies momentum to obtain an intermediate point
\(y_{n+1}\), then evaluates the gradient at this intermediate point \(y_{n+1}\)
instead of \(\param_n\).
% \[
% 	y_{n+1} = \param_n + \beta_n(\param_n - \param_{n-1})
% 	\quad\text{and}\quad
% 	\param_{n+1} = y_{n+1} - \stepsize_n \nabla\Cost(y_{n+1}).
% \]
This procedure is guaranteed to converge on convex functions with
\(L\)-Lipschitz gradient with optimal rate \(\bigO(1/n^2)\) for certain
selections of \(\beta_n, \stepsize_n\)
\citep{nesterovLecturesConvexOptimization2018}. Since optimization
on a random function will eventually enter a convex area, this is a plausible
assumption for the asymptotic behavior.
We take inspiration from the conservative infinite condition case without strong
convexity (\(\mu=0\)). The recursion for \(\beta_n\) from the Constant Step
Scheme II \citep[93]{nesterovLecturesConvexOptimization2018} is then well
approximated by
\[
	\stepsize_n = \tfrac1L \quad\text{and} \quad \beta_n = \tfrac{n-1}{n+2}.
\]
Since \(\beta_n\) is explicit here, only a step size \(\stepsize_n\) is required to
define random function momentum. Inspired by the optimal step size of gradient
descent in the strongly convex case \citep{gohWhyMomentumReally2017}
\[
	\stepsize_n = \tfrac{2}{L+\mu} \overset{\mu=0}= \tfrac{2}L,
\]
and Example~\ref{ex: gradient descent} we halved the step size suggested by
\ref{rfd}, which results in the performance improvement we call
\rfm{} (Figure~\ref{fig: condition and rfm}). The \(*\)
emphasizes the educated guess involved.

% \begin{algorithm*}[H]\label{algo: rfm}
% 	\caption{S\rfm{}}
% 	Estimate the parameters of a covariance model \(\sqC\) and sample
% 	variance \(\E[\epsilon_0^2]\) and \(\E[\epsilon_1\epsilon_1^T]=\sigma^2\identity\)\;
% 	\(
% 	c \leftarrow \tfrac{\sqC(0)}{\sqC(0) + \E[\sigma_0^2]}
% 	\tfrac{\sigma^2 - \sqC'(0)}{-\sqC'(0)}
% 	\)\tcp*{=1 in \rfm{} with full gradients}
% 	\KwIn{starting point \(\param\)}
% 	\(\param_{\text{prev}} \leftarrow \param\); \(n\leftarrow 1\)\;
% 	\While{not converged}{
% 		\(\beta \leftarrow \frac{n-1}{n+1}\); \(n\leftarrow n+1\)
% 		\tcp*{\(\beta=0\) for RFD}
% 		\(
% 			y \leftarrow \param + \beta(\param - \param_{\text{prev}})
% 		\)\tcp*{Momentum Step}
% 		\(\param_{\text{prev}}\leftarrow \param\);
% 		\(Z \leftarrow\) minibatch of dataset
% 		\tcp*{Update \(c\) if batch size changes}
% 		\(\Theta \leftarrow c \frac{\loss(\param,Z)-\mu}{\|A^{-1}\grad\loss(\param, \tilde{Z})\|_A}\);
% 		\(\stepsize \leftarrow
% 			\argmin_{\stepsize} \frac{\sqC(\stepsize^2)}{\sqC(0)}\Theta - \stepsize \frac{\sqC'(\stepsize^2)}{\sqC'(0)}
% 		\)
% 		\tcp*{cf.~Subsection~\ref{sec: optimal step-size}}
% 		\(
% 			\param \leftarrow y - \frac{\stepsize}{\color{red} 2} \nabla \loss(y, Z)
% 		\)
% 		\tcp*{do not divide step size by two for RFD}
% 	}
% \end{algorithm*}	



==> sections/extensions/linear_isotropy/asymptotic_rfd.tex <==
\subsection{Asymptotic RFD and Convergence}

In this subsection we discuss an approximation to the step sizes of RFD which
becomes asymptotically correct as the gradient norm vanishes. There are two
reasons why this is useful. The first is that we avoid the use of a
specific covariance model and thus will be able to estimate the approximate
step sizes non-parametrically (Sec.~\ref{sec: stochastic loss and covariance
estimation}). The second reason is that we can use the asymptotic correctness
to argue that RFD can only converge to stationary points (Theorem~\ref{thm:
convergence to stationary point}).

Recall that the step sizes \((h^*, \stepsize^*)\) suggested by RFD are the minimizer
of \(q(h,\stepsize)\) from Theorem~\ref{thm: rfd reduces to gradient descent}. As
we expect step sizes to converge to \(0\), the minimizer of the 2\textsuperscript{nd} Taylor
expansion of \(q\) should be asymptotically accurate (Conjecture~\ref{conj: A-RFD asymptotically equal RFD}).
We can prove this conjecture formally for the squared exponential covariance
(Prop.~\ref{prop: A-RFD for squared exponential covariance}) and graphically for
the remaining examples in Table~\ref{table: optimal step size}
(Appendix~\ref{subsec: proof sketch conjecture}).

\begin{definition}[Asymptotic RFD]
	For \(\step\) and \(q\) as in Theorem~\ref{thm: rfd reduces to gradient
	descent} we call
	\[
		\param_{n+1} := \param_n - \tilde{\step}
		\quad\text{with}\quad
		\tilde{\step} := \step(\tilde{h}, \tilde{\stepsize})
	\]
	Asymptotic RFD (A-RFD) with step sizes
	\[
		\begin{pmatrix}
			\tilde{h}\\ \tilde{\stepsize}
		\end{pmatrix}
		:= - [\nabla^2 q(0,0)]^{-1} \nabla q(0,0).
	\]
\end{definition}

\begin{conjecture}\label{conj: A-RFD asymptotically equal RFD}
	If either \((h^*, \stepsize^*)\to 0\) or \((\tilde{h}, \tilde{\stepsize})\to 0\), then
	the step sizes of asymptotic RFD and RFD are asymptotically equal
	\[
		(h^*, \stepsize^*) \sim (\tilde{h}, \tilde{\stepsize})
	\quad\text{i.e.}\quad
		\tfrac{\tilde{h}}{h} \to 1
		\quad\text{and}\quad
		\tfrac{\tilde{\stepsize}}{\stepsize} \to 1.
	\]
\end{conjecture}

\begin{prop}[Tayloring the Conditional Expectation]
    \label{prop: tayloring the conditional expectation}
    In the setting of Theorem~\ref{thm: rfd reduces to gradient descent}, the
    second order Taylor expansion of \(q\) around zero is given by
    \begin{align*}
        q(0,0) &= \magenta{\Cost(x)}
        \\
        \nabla q(0,0) &= -\begin{pmatrix}
            \teal{D_{\hat{x}}\Cost(x)}
            \\
            \teal{\|\proj{x^\perp}\nabla\Cost(x)\|}
        \end{pmatrix}\\
        \nabla^2q(0,0) &= \begin{pmatrix}
			a & c
			\\
			c & b
		\end{pmatrix}
    \end{align*} 
    where for \(\mu_\Cost(x) = \mu\bigl(\tfrac{\|x\|^2}2\bigr)\)
    \begin{align*}
        a &= \begin{aligned}[t]
			&\begin{pmatrix}
				\C_\Cost(x,D_{\hat{x}}^2x)
				\\
				\blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}^2x)}
			\end{pmatrix}^T 
			\! \Sigma^{-1}
			\begin{pmatrix}
				\magenta{\bar{\Cost}(x)}
				\\
				\teal{D_{\hat{x}}\bar{\Cost}(x)}
			\end{pmatrix}
			\\
			&+ \mu''\bigl(\tfrac{\|x\|^2}2\bigr)\|x\|^2 + \mu'\bigl(\tfrac{\|x\|^2}2\bigr)
		\end{aligned}
        \\
        b &= \begin{pmatrix}
            \C_\Cost(x,D_{\hat{\prgrad}}^2x)
            \\
            \blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{\prgrad}}^2x)}
        \end{pmatrix}^T 
        \! \Sigma^{-1}
        \begin{pmatrix}
            \magenta{\bar{\Cost}(x)}
            \\
            \teal{D_{\hat{x}}\bar{\Cost}(x)}
        \end{pmatrix}
        + \mu'\bigl(\tfrac{\|x\|^2}2\bigr)
		\\
		c &=\frac{
			\blue{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{x}}D_{\hat{\prgrad}}x)}
		}{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)}
		\teal{\bigl\|\proj{x^\perp}\nabla\Cost(x)\bigr\|}.
    \end{align*}
    In the \textbf{(affine) isotropic} case the Hessian reduces to
    \[
        \nabla^2q(0,0) = \tfrac{\ikernel_\Cost'(0)}{\ikernel_\Cost(0)}\magenta{\bar{\Cost}(x)} \identity.
    \]
\end{prop}


\begin{corollary}[A-RFD in the Affine Isotropic Case]\label{cor: a-rfd in the affine isotropic case}
	\[
		\tilde{\step}
		= \frac{\ikernel_\Cost(0)}{\ikernel_\Cost'(0)\magenta{\bar{\Cost}(x)}} \teal{\nabla\Cost(x)}
		= \frac{\ikernel_\Cost(0)}{-\ikernel_\Cost'(0)(\mu-\magenta{\Cost(x)})} \teal{\nabla\Cost(x)}.
	\]
\end{corollary}
Step size selection would therefore only require non-parametric estimation of
\(\ikernel_\Cost(0),\ikernel_\Cost'(0)\) and the mean \(\mu\).

\begin{theorem}[Convergence to Stationary Points]
	\label{thm: convergence to stationary point}
	In the isotropic case A-RFD can only converge to stationary points. If
	Conjecture~\ref{conj: A-RFD asymptotically equal RFD} holds, the same is true for RFD.
\end{theorem}
\begin{proof}
	If the parameters \(\param_n\) induced by A-RFD converge to some \(\param_\infty\), then
	continuity of \(\Cost\) implies \(\Cost(\param_n)\to\Cost(\param_\infty)\). As \(\param_n\)
	is a Cauchy sequence and \(\tilde{\step}_n = \param_{n+1} -\param_n\) we have
	\[
		\|\nabla\Cost(\param_\infty)\| \leftarrow \|\nabla\Cost(\param_n)\|
		= \bigl|\tfrac{\ikernel_\Cost'(0)\magenta{\bar{\Cost}(\param_n)}}{\ikernel_\Cost(0)}\bigr| \|\tilde{\step}_n\| \to 0.
		\qedhere
	\]
\end{proof}
\begin{example}
	Conjecture~\ref{conj: A-RFD asymptotically equal RFD} holds for the squared exponential covariance
	(Prop.~\ref{prop: A-RFD for squared exponential covariance}). So when the
	loss has this covariance, RFD can only converge to stationary points.
\end{example}

This does not quite prove convergence and only covers the affine isotropic case.
The classical analysis of gradient descent uses step sizes small enough to
guarantee an improvement in every step. This makes it much easier to prove
convergence than it is for RFD where the step sizes are optimal on average. But
at the same time convergence proofs for RFD will be much more meaningful, as the
step sizes are actually realistic in practice.

The key ingredient in the convergence proof is the fact that step sizes are
asymptotically proportional to the gradient norm. We can uncover a similar relationship
in the \emph{linear} isotropic case under the assumption \(\|\nabla\Cost(\param_n)\|\to 0\)
(Proposition~\ref{prop: asymptotic approx optimal step}). Since this would
make a convergence proof cyclic, more research is needed to excavate this
relationship without this assumption.

==> sections/extensions/linear_isotropy/covariance_of_derivatives.tex <==
\subsection{Covariance of Derivatives}\label{sec: covariance of derivatives}


\begin{lemma}[Taylor Covariance]
	\label{lem: taylor covariance}
	For a random function \(\rf\) with 
	\[
		\C_{\rf}(x,y)
		= \kernel\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr),
	\]
	using the short notation
	\[
		\kernel_i(t_1,t_2,t_3) = \frac{d}{dt_i}\kernel(t_1,t_2,t_3) \quad \text{etc.}
	\]
	and
	\[
		\kernel = \kernel\bigl(\tfrac{\|x\|^2}2, \tfrac{\|x\|^2}2, 0\bigr),
	\]
	we have
	\begin{align}
		\label{eq: taylor cov - (Dv x, x)}
		&\C_{\rf}(D_v x, x) 
		= \kernel_1 \langle x, v\rangle
		\\
		\label{eq: taylor cov - (Dv x, Dw x)}
		&\C_{\rf}(D_v x, D_w x)
		= \kernel_{12} \langle x, v\rangle\langle x, w\rangle - \kernel_3\langle v, w\rangle
		\\
		\label{eq: taylor cov - (Dv1 Dv2 x, x)}
		&\C_{\rf}(D_{v_1}D_{v_2} x, x)
		\\ \nonumber
		&= \kernel_{11} \langle x, v_1\rangle\langle x, v_2\rangle + (\kernel_1+\kernel_3)\langle v_1, v_2\rangle
		\\
		\label{eq: taylor cov - (Dv x, Dw1 Dw2 x)}
		&\C_{\rf}(D_v x, D_{w_1}D_{w_2}x)
		\\ \nonumber
		&=\begin{aligned}[t]
			&\kernel_{122}\langle x, v\rangle\langle x, w_1\rangle\langle x, w_2\rangle
			+ (\kernel_{12} + \kernel_{13})\langle x,v\rangle\langle w_1, w_2\rangle
			\\
			&-\kernel_{23}\Bigl(
				\langle v, w_2\rangle\langle x, w_1\rangle
				+ \langle v, w_1\rangle\langle x, w_2\rangle
			\Bigr)
		\end{aligned}
	\end{align}

\end{lemma}
\begin{proof}
	We carefully take partial derivatives	
	\begin{equation}
		\label{eq: lin isotropic covariance first derivative}
		\C_{\rf}(D_v x, y)
		= \begin{aligned}[t]
			&\kernel_1\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr)\langle x, v\rangle 
			\\
			&+ \kernel_3\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr)\langle x-y, v\rangle
		\end{aligned}
	\end{equation}
	This already leads to the first claim. But we continue to take derivatives to get
	\begin{align*}
		&\C_{\rf}(D_{v_1}D_{v_2}x, y)
		\\
		&= \begin{aligned}[t]
			&\kernel_{11}\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr)
			\langle x, v_1\rangle\langle x, v_2\rangle
			\\
			&- \kernel_{13}\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr)
			\langle x, v_1\rangle\langle y-x, v_2\rangle
			\\
			&+ \kernel_1\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr)\langle v_1,v_2\rangle
			\\
			&- \kernel_{31}\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr)
			\langle y-x, v_1\rangle\langle x, v_2\rangle
			\\
			&+ \kernel_{33}\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr)
			\langle y-x, v_1\rangle\langle y-x, v_2\rangle
			\\
			&+ \kernel_3\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr)
			\langle v_1, v_2\rangle.
		\end{aligned}
	\end{align*}
	Taking the derivative in the other position results in
	\begin{align*}
		&\C_{\rf}(D_v x, D_w y)
		\\
		&= \begin{aligned}[t]
			&\kernel_{12}\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr)\langle x, v\rangle \langle y, w\rangle
			\\
			&+ \kernel_{13}\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr)\langle y-x, w\rangle\langle x, v\rangle
			\\
			&- \kernel_{23}\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr) \langle y-x, v\rangle\langle y, w\rangle
			\\
			&- \kernel_{33}\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr) \langle y-x, v\rangle \langle y-x, w\rangle
			\\
			&- \kernel_3\bigl(\tfrac{\|x\|^2}2, \tfrac{\|y\|^2}2, \tfrac{\|y-x\|^2}2\bigr)\langle v, w\rangle
		\end{aligned}
		\\
		\overset{x=y}&=
		\begin{aligned}[t]
			&\kernel_{12}\bigl(\tfrac{\|x\|^2}2, \tfrac{\|x\|^2}2, 0\bigr)\langle x,v\rangle \langle y, w\rangle
			\\
			&- \kernel_3\bigl(\tfrac{\|x\|^2}2, \tfrac{\|x\|^2}2, 0\bigr)\langle v, w\rangle
		\end{aligned}
	\end{align*}
	We leave the last claim as an exercise to save space. Note that whenever
	\(y-x\) appears in a product, it needs to go away (otherwise it would be set to
	zero when \(x=y\)), so in the product rule we can skip the other places with \(y\).
\end{proof}


==> sections/extensions/linear_isotropy/general_rfd.tex <==
\section{Appendix: Random Function Descent}

Before we state our result connecting RFD to gradient descent, we introduce some
notation. We use hat notation \(\hat{\cdot}\) for normalization
(i.e. \(\hat{y} = \frac{y}{\|y\|}\)). \(\proj{x^\perp}\) is the projection to
the orthogonal space \(x^\perp\) of \(x\). And we define
\begin{align}
    \bar{\Cost} &:= \Cost - \mu_\Cost
	 \nonumber
    \\
    \Sigma
    &:= \Cov\Bigl(\begin{pmatrix}
        \Cost(x)\\ D_{\hat{x}}\Cost(x)
    \end{pmatrix}\Bigr) \in \real^{2\times 2}
	 \label{eq: sigma definition}
    \\
    \prgrad &:= \proj{x^\perp}\nabla\Cost(x),
	 \nonumber
\end{align}
where \(D_v f\) is the directional derivative of \(f\) in the direction of \(v\).
We further use the notation \(f(D_v x) := D_v f(x)\), i.e.
\begin{align*}
    \C_\Cost(D_v x,y)
	&:= \tfrac{d}{dt}\C_\Cost(x + tv, y)\Bigr|_{t=0}
	\\
	\overset{(*)}&= \Cov(D_v \Cost(x), \Cost(y)).
\end{align*}
For \((*)\) we swap differentiation with integration.\footnote{
	For a centered random function \(\rf\) we have
	\[
		\partial_{x_i}\C_{\rf}(x,y)
		= \partial_{x_i} \E[\rf(x) \rf(y)]
		= \Cov(\partial_{x_i}\rf(x), \rf(y))
	\]
	So differentiability of the covariance function is certainly necessary for
	\(\partial_{x_i}\rf\) to exist and almost sufficient
	\citep[details in][Sec.~1.4.2]{adlerRandomFieldsGeometry2007}.
	It is likely that many results could be generalized to derivatives in the sense
	of distributions. One could take a closer look at differentiability viewed through
	this lens in the future.
	Since \(\prgrad\) is a random variable, we finally want to caution
	\[
		\C_\Cost(D_{\hat{\prgrad}}x, y)
		\overset{\text{in general}}\neq \Cov(D_{\hat{\prgrad}} \Cost(x), \Cost(y)).
	\]
}

\begin{theorem}[RFD Reduces to Gradient Descent]
	\label{thm: rfd reduces to gradient descent}
	Assume that \(\Cost\) is a \textbf{non-stationary isotropic} Gaussian random function. Then
	a gradient-like step
	\[
		\step(h,\stepsize)
		= h \hat{x}
		+ \stepsize \hat{\prgrad}
	\]
	minimizes the conditional expectation
	\[
		\min_{\step\in\real^\dims} \E[\Cost(x-\step)\mid \Cost(x),\nabla\Cost(x)]
		= \min_{h,\stepsize\in\real}
		\underbrace{
			\E\bigl[\Cost\bigl(x-\step(h,\stepsize)\bigr) \mid \Cost(x),\nabla\Cost(x)\bigr]
		}_{=: q(h, \stepsize)}.
	\]
    And the optimal step sizes are the minimizer of
    \[
        q(h,\stepsize)
        = \begin{pmatrix}
				\C_\Cost(x,x-\step)
				\\
				\C_\Cost(D_{\hat{x}}x, x-\step)
			\end{pmatrix}^T 
			\!\Sigma^{-1}\!
			\begin{pmatrix}
				\magenta{\bar{\Cost}(x)}
				\\
				\teal{D_{\hat{x}}\bar{\Cost}(x)}
			\end{pmatrix}
			+ \frac{\C_\Cost(D_{\hat{\prgrad}}x, x-\step)}{
				\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)
			}
			\teal{\bigl\|\prgrad\bigr\|} + \mu_\Cost(x-\step),
    \]
    where we omitted the inputs to the step \(\step = \step(h,\stepsize)\) for brevity.

    If \(\Cost\) is \textbf{(affine) isotropic} with covariance function
    \[
		\C_\Cost(x,y) = \ikernel_\Cost\bigl(\tfrac{\|y-x\|^2}2\bigr),
	\]
	then the gradient step
    \[
        \step(\stepsize) = \stepsize \tfrac{\nabla\Cost(x)}{\|\nabla\Cost(x)\|}
    \]
    minimizes the conditional expectation
    \begin{align*}
        \min_{\step\in \real^\dims} \E[\Cost(x-\step)\mid \Cost(x), \nabla\Cost(x)]
        = \min_{\stepsize} \E[\Cost(x-\step(\stepsize))\mid \Cost(x),\nabla\Cost(x)]
	\end{align*}
    and the optimal step size is given by
    \[
        \stepsize^*
        = \argmin_{\stepsize} \tfrac{\ikernel_\Cost(\frac{\stepsize^2}2)}{\ikernel_\Cost(0)} \magenta{\bar{\Cost}(x)}
        - \stepsize\tfrac{\ikernel_\Cost'(\frac{\stepsize^2}2)}{\ikernel_\Cost'(0)}\teal{\|\nabla\Cost(x)\|}.
    \]
\end{theorem}

\subsection{Proof of Theorem~\ref{thm: rfd reduces to gradient descent}}


We recommend preparing a copy of Lemma~\ref{lem: taylor covariance} (where we calculated
derivatives of the covariance function) as a reference for this proof, since we will make repeated use
of it.

\textbf{Calculating the conditional Expectation:} 
By Theorem~\ref{thm: characterization of weak input invariances} we can
assume without loss of generality that the covariance function of a non-stationary
isotropic random function is of the form
\[
	 \C_\Cost(x,x+\step)
	 = \kernel\bigl(\tfrac{\|x\|^2}2, \tfrac{\|x-\step\|^2}2, \tfrac{\|\step\|^2}2\bigr)
\]
and the mean of the form \(\mu_\Cost(x) = \mu\bigl(\frac{\|x\|^2}2\bigr)\)
and use the notation
\begin{enumerate}
	 \item \(\kernel[\step] = \kernel\bigl(\tfrac{\|x\|^2}2, \tfrac{\|x-\step\|^2}2, \tfrac{\|\step\|^2}2\bigr)\)
	 \item \(\kernel=\kernel[0]\) and
	 \item \(\kernel_i(t_1,t_2,t_3) = \frac{d}{dt_i}\kernel(t_1,t_2,t_3)\) and similarly for higher order derivatives.
\end{enumerate}
The formula for the conditional expectation of joint Gaussian random variables is well known to be
\begin{align*}
	 &\E[\Cost(x-\step) \mid \Cost(x), \nabla\Cost(x)]
	 \\
	 &=
		\Cov\Bigl(
		  \begin{pmatrix}
				\Cost(x)\\
				\nabla\Cost(x)
		  \end{pmatrix},
		  \Cost(x-\step)
	 \Bigr)^T
	 \Bigl[\Cov\Bigl(\begin{pmatrix}
		  \Cost(x)\\
		  \nabla\Cost(x)
	 \end{pmatrix}\Bigr)\Bigr]^{-1}
	 \begin{pmatrix}
		  \magenta{\bar{\Cost}(x)}
		  \\
		  \teal{\nabla\bar{\Cost}(x)}
	 \end{pmatrix}
	 + \mu_\Cost(x-\step).
\end{align*}
We now choose an orthonormal basis \((e_i)_i\) with \(e_1 = \hat{x}\) with
regard to which, we write vector and matrix entries. Recalling the definition
\eqref{eq: sigma definition} of \(\Sigma\), We have by Section~\ref{sec:
covariance of derivatives} in particular \eqref{eq: taylor cov
- (Dv x, x)} and \eqref{eq: taylor cov - (Dv x, Dw x)}
\[
	 \Cov\Bigl(
		  \begin{pmatrix}
				\Cost(x)\\
				\nabla\Cost(x)
		  \end{pmatrix}
	 \Bigr)
	 = \left(\begin{array}{c  c} 
		  \Sigma &
		  \\
		  & - \kernel_3 \identity_{\dims-1}
	 \end{array}
	 \right).
\]
Inverting the blocks individually we get
\[
	 \Bigl[\Cov\Bigl(
		  \begin{pmatrix}
				\Cost(x)\\
				\nabla\Cost(x)
		  \end{pmatrix}
	 \Bigr)\Bigr]^{-1}
	 = \left(\begin{array}{c c}
		  \Sigma^{-1}
		  \\
		  & - 1/\kernel_3 \identity_{\dims-1}
	 \end{array}
	 \right).
\]
We have by \eqref{eq: lin isotropic covariance first derivative} in the proof of Lemma~\ref{lem: taylor covariance}
\[
	 \Cov\Bigl(
		  \begin{pmatrix}
				\Cost(x)\\
				\nabla\Cost(x)
		  \end{pmatrix},
		  \Cost(x-\step)
	 \Bigr)
	 = \begin{pmatrix}
		  \C_\Cost(x, x-\step)
		  \\
		  \C_\Cost(D_{\hat{x}} x, x-\step)
		  \\
		  \top
		  \\
	 \kernel_3[ \step ] \proj{x^\perp}(\step)
	 \\
	 \bot
	 \end{pmatrix}
\]
where we view \(\proj{x^\perp}(\step)\in \real^\dims\)  as a member of \(\real^{\dims-1}\) since the first
entry is the direction \(e_1 = \hat{x}\) which is (by defnition of \(\proj{x^\perp}\)) always zero.
Since
\[
	 \nabla\bar{\Cost}(x)
	 = \nabla\Cost(x) - \mu\bigl(\tfrac{\|x\|^2}2\bigr) = \nabla\Cost(x) - \mu'\bigl(\tfrac{\|x\|^2}2\bigr)x
\]
we have
\begin{align}
	 \label{eq: Dx L(x)}
	 D_{\hat{x}}\bar{\Cost}(x) 
	 &= D_{\hat{x}}\Cost(x) - \mu'\bigl(\tfrac{\|x\|^2}2\bigr)\|x\|
	 \\
	 \label{eq: Px grad L(x)}
	 \proj{x^\perp}\nabla\bar{\Cost}(x)
	 &= \proj{x^\perp}\nabla\Cost(x).
\end{align}
I.e. the gradient on the orthogonal complement of \(x\) is unaffected by centering.
Putting things together, we get
\begin{align*}
	 &\E[\Cost(x-\step) \mid \Cost(x), \nabla\Cost(x)]
	 \\
	 &= \begin{pmatrix}
				\C_\Cost(x, x-\step)
				\\
				\C_\Cost(D_{\hat{x}} x, x-\step)
		  \end{pmatrix}^T \Sigma^{-1}\begin{pmatrix}
				\magenta{\bar{\Cost}(x)}\\
				\teal{D_{\hat{x}}\bar{\Cost}(x)}
		  \end{pmatrix}
		  - \frac{\kernel_3[\step]}{\kernel_3}\bigl\langle \proj{x^\perp}(\step), \teal{\proj{x^\perp}\nabla\Cost(x)}\bigr\rangle
		  + \mu_\Cost(x-\step).
\end{align*}

\textbf{Addendum for affine isotropy:} In the case of affine isotropy, it is
not difficult to see (referencing Lemma~\ref{lem: taylor covariance} \eqref{eq: taylor cov - (Dv x, x)}) that
\(\Sigma\) is a diagonal matrix, since
\[
	 \C_\Cost(x,x-\step) = \ikernel\bigl(\tfrac{\|\step\|^2}2\bigr)
	 \Bigl( = \kernel\bigl(\tfrac{\|x\|^2}2, \tfrac{\|x-\step\|^2}2, \tfrac{\|\step\|^2}2\bigr)\Bigr)
\]
implies \(\kernel_1 \equiv \kernel_2 \equiv 0\) as the covariance only
depends on the third input. And the mean is constant
(\(\mu\bigl(\tfrac{\|x\|^2}2\bigr)=\mu\)) and thus \(\mu'=0\). Putting
things together we get
\begin{align*}
	\E[\Cost(x-\step) \mid \Cost(x), \nabla\Cost(x)]
	= \frac{\ikernel\bigl(\frac{\|\step\|^2}2\bigr)}{\ikernel(0)}
	\magenta{\bar{\Cost}(x)}
	- \frac{\ikernel'\bigl(\frac{\|\step\|^2}2\bigr)}{\ikernel'(0)}\bigl\langle \step, \teal{\nabla\Cost(x)}\bigr\rangle
	+ \mu.
\end{align*}

\textbf{Minimization:} To understand the method we want to apply, it is instructive to start out
with the affine isotropic case. So we prove this case first: We split the minimization task into
step size and direction
\begin{align*}
	\min_{\step\in \real^\dims}\E[\Cost(x-\step)\mid \Cost(x), \nabla\Cost(x)]
	= \min_{\stepsize \ge 0} \min_{\substack{v \in \real^\dims\\ \|v\|=1}}
	\E[\Cost(x-\stepsize v)\mid \Cost(x), \nabla\Cost(x)].
\end{align*}
Using our representation of the expectation, we note there is only one place, where the direction
actually matters
\begin{align*}
	\min_{\substack{v \in \real^\dims\\ \|v\|=1}}\E[\Cost(x-\stepsize v) \mid \Cost(x), \nabla\Cost(x)]
	= \min_{\substack{v \in \real^\dims\\ \|v\|=1}}\frac{\ikernel\bigl(\frac{\stepsize^2}2\bigr)}{\ikernel(0)}
	\magenta{\bar{\Cost}(x)}
	- \stepsize\frac{\ikernel'\bigl(\frac{\stepsize^2}2\bigr)}{\ikernel'(0)}\bigl\langle v, \teal{\nabla\Cost(x)}\bigr\rangle
	+ \mu.
\end{align*}
So we need to either maximize or minimize \(\langle v,
\nabla\Cost(x)\rangle\), depending on the sign of
\(\frac{\ikernel'(\stepsize^2/2)}{\ikernel'(0)}\). Up to the sign
the result is therefore by Lemma~\ref{lem: constrained maximiziation of
scalar products} and Corollary~\ref{cor: constrained minimization of scalar products}
\[
	 v^* = \pm \frac{\nabla\Cost(x)}{\|\nabla\Cost(x)\|}.
\]
Common sense dictates the sign should be positive (otherwise we would move up the
gradient). But since we restricted \(\stepsize\) to be positive in the outer
minimization and only \(\stepsize^2\) appears in the formula, except for the place
we are considering, we can simply avoid this problem by letting \(\stepsize\) be any
real number. This results in
\begin{align*}
	\min_{\step\in \real^\dims}\E[\Cost(x-\step)\mid \Cost(x), \nabla\Cost(x)]
	= \min_{\stepsize \in \real} 
	\E[\Cost(x-\step(\stepsize))\mid \Cost(x), \nabla\Cost(x)].
\end{align*}
with
\[
	 \step(\stepsize) = \stepsize\frac{\nabla\Cost(x)}{\|\nabla\Cost(x)\|}.
\]
and the optimal step size is the minimizer of
\begin{align*}
	\E[\Cost(x-\step(\stepsize))\mid \Cost(x), \nabla\Cost(x)]
	= \frac{\ikernel\bigl(\frac{\stepsize^2}2\bigr)}{\ikernel(0)}
	\magenta{\bar{\Cost}(x)}
	- \stepsize\frac{\ikernel'\bigl(\frac{\stepsize^2}2\bigr)}{\ikernel'(0)} \teal{\|\nabla\Cost(x)\|}
	+ \mu.
\end{align*}
The constant \(\mu\) does not matter for minimization, so we leave it out in the theorem.

\textbf{Minimization in the non-stationary isotropic case:} The trick is the same, we just have to treat the
direction \(\hat{x}\) separately, and the formulas are larger. I.e.
\begin{align*}
	 &\min_{\step\in \real^\dims} \E[\Cost(x+\step) \mid \Cost(x), \nabla\Cost(x)]
	 \\
	 &= \min_{h\in\real} \min_{\stepsize\ge 0} \min_{\substack{v\in x^\perp\\ \|v\|=1}}
	 \E\Bigl[\Cost\Bigl(x - \step(h, \stepsize, v)\Bigr) \mid \Cost(x), \nabla\Cost(x)\Bigr]
\end{align*}
with
\[
	 \step = \step(h, \stepsize, v) = h \hat{x} + \stepsize v.
\]
Notice how we restricted \(v\) to be in the orthogonal space of \(x\) this time. This implies both
\begin{align}
	 \label{eq: |d| = h^2 + eta^2}
	 \|\step\|^2 
	 &= h^2 + \stepsize^2, \quad \text{and}
	 \\
	 \label{eq: |x-d| = |x|^2 - 2h|x| + h^2 + eta^2}
	 \|x-\step\|^2
	 &= \bigl(1-\tfrac{h}{\|x\|}\bigr)^2 \|x\|^2 + \stepsize^2
	 \\
	 \nonumber
	 &= \|x\|^2 -2h\|x\| + h^2 + \stepsize^2
\end{align}
are constant in \(v\). Since these are the inputs of \(\kernel\) it is
perhaps not difficult to see, where this is going. We now have
\begin{align*}
	&\E[\Cost(x-\step) \mid \Cost(x), \nabla\Cost(x)]
	\\
	&= 
	\begin{pmatrix}
		\C_\Cost(x, x-\step)
		\\
		\C_\Cost(D_{\hat{x}} x, x-\step)
	\end{pmatrix}^T \Sigma^{-1}\begin{pmatrix}
		\magenta{\bar{\Cost}(x)}\\
		\teal{D_{\hat{x}}\bar{\Cost}(x)}
	\end{pmatrix}
	- \stepsize\frac{\kernel_3[\step]}{\kernel_3}\bigl\langle v, \teal{\proj{x^\perp}\nabla\Cost(x)}\bigr\rangle
	+ \mu\bigl(\tfrac{\|x-\step\|^2}2\bigr).
\end{align*}
With the second line in the form we want, we merely need to show that the first line is constant in \(v\).
For this we reference Lemma~\ref{lem: taylor covariance} again. We have
\begin{align*}
	 \C_\Cost(x, x-\step) 
	 \overset{\text{def.}}&= \kernel[\step]
	 \\
	 \C_\Cost(D_{\hat{x}}x, x-\step)
	 \overset{\eqref{eq: lin isotropic covariance first derivative}}&=
	 \kernel_1[\step]\underbrace{\langle x, \hat{x}\rangle}_{=\|x\|} + \kernel_3[\step]\underbrace{\langle \step, \hat{x}\rangle}_{=h}
\end{align*}
The entries of \(\Sigma\) are independent of \(\step\) and thus also of \(v\).
With the same trick we now get
\[
	 d(h, \stepsize) = h \hat{x} + \stepsize \hat{\prgrad}
\]
where \(\prgrad = \proj{x^\perp}\nabla\Cost(x)\) and the remaining function
in \(h, \stepsize\) is given by
\[
	 \begin{pmatrix}
		  \C_\Cost(x, x-\step)
		  \\
		  \C_\Cost(D_{\hat{x}} x, x-\step)
	 \end{pmatrix}^T \Sigma^{-1}\begin{pmatrix}
		  \magenta{\bar{\Cost}(x)}\\
		  \teal{D_{\hat{x}}\bar{\Cost}(x)}
	 \end{pmatrix}
	 \qquad - \stepsize\frac{\kernel_3[\step]}{\kernel_3}\teal{\|\proj{x^\perp}\nabla\Cost(x)\|}
	 + \mu\bigl(\tfrac{\|x-\step\|^2}2\bigr).
\]
Using Lemma~\ref{lem: taylor covariance} one last time, we note
\begin{align*}
	 \C_\Cost(D_{\hat{\prgrad}}x, x-\step)
	 \overset{\eqref{eq: lin isotropic covariance first derivative}}&=
	 \kernel_3[\step]\langle \step, \hat{\prgrad}\rangle 
	 = \kernel_3[\step]\stepsize
	 \\
	 \C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)
	 \overset{\eqref{eq: taylor cov - (Dv x, Dw x)}}&= -3\kernel_3
\end{align*}
Putting things together, we get the claim about \(q\).

\subsection{Proof of Proposition~\ref{prop: tayloring the conditional expectation}}

First of all we have
\begin{align*}
	 q(0,0)
	 &= 
		\underbrace{\begin{pmatrix}
		  \C_\Cost(x,x)
		  \\
		  \C_\Cost(D_{\hat{x}}x, x)
	 \end{pmatrix}^T 
	 \Sigma^{-1}
	 }_{= \begin{pmatrix}1 & 0\end{pmatrix}}
	 \begin{pmatrix}
		  \magenta{\bar{\Cost}(x)}
		  \\
		  \teal{D_{\hat{x}}\bar{\Cost}(x)}
	 \end{pmatrix}
	 + \underbrace{
		  \frac{\C_\Cost(D_{\hat{\prgrad}}x, x)}{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)}
	 }_{\overset{\eqref{eq: taylor cov - (Dv x, x)}}=0}
	 \teal{\bigl\|\prgrad\bigr\|} + \mu_\Cost(x)
	 \\
	 &= \magenta{\Cost(x)},
\end{align*}
since the vector in front coincides with the first column of \(\Sigma\).
Using the expression for \(\|x-\step\|^2\) in \eqref{eq: |x-d| = |x|^2 -
2h|x| + h^2 + eta^2} we take the derivative with respect to \(h\)
\begin{align*}
	&\frac{d}{dh}q(h,\stepsize)
	\\
	&= \begin{aligned}[t]
		  &-\begin{pmatrix}
				\C_\Cost(x,D_{\hat{x}}(x-\step))
				\\
				\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}(x-\step))
		  \end{pmatrix}^T 
		  \Sigma^{-1}
		  \begin{pmatrix}
				\magenta{\bar{\Cost}(x)}
				\\
				\teal{D_{\hat{x}}\bar{\Cost}(x)}
		  \end{pmatrix}
		  \\
	 &- \frac{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{x}}(x-\step))}{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)}
		  \teal{\bigl\|\prgrad\bigr\|}
	\\
	 &+ \mu'\bigl(\tfrac{\|x-\step\|^2}2\bigr)(-\|x\| + h)
	 \end{aligned}
\end{align*}
and thus
\begin{align*}
	 \frac{d}{dh}q(0,0)
	 &= \begin{aligned}[t]
		&-\underbrace{\begin{pmatrix}
				\C_\Cost(x,D_{\hat{x}}x)
				\\
				\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}x)
		  \end{pmatrix}^T 
		  \Sigma^{-1}
	 }_{=\begin{pmatrix}0 & 1\end{pmatrix}}
		  \begin{pmatrix}
				\magenta{\bar{\Cost}(x)}
				\\
				\teal{D_{\hat{x}}\bar{\Cost}(x)}
		  \end{pmatrix}
		  \\
	 &\quad - \underbrace{
		  \frac{
				\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{x}}x)
		  }{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)}
	 }_{\overset{\eqref{eq: taylor cov - (Dv x, Dw x)}}=0}
	 \teal{\bigl\|\prgrad\bigr\|}
	 - \mu'\bigl(\tfrac{\|x\|^2}2\bigr)\|x\|
		\end{aligned}
	 \\
	 &= -\teal{D_{\hat{x}}\bar{\Cost}(x)} - \mu'\bigl(\tfrac{\|x\|^2}2\bigr)\|x\|
	 \\
	 \overset{\eqref{eq: Dx L(x)}}&= -\teal{D_{\hat{x}}\Cost(x)},
\end{align*}
where we use that the vector in front coincides with the second column of \(\Sigma\). Similarly
we can take the derivative with respect to \(\stepsize\), to get
\begin{align*}
	 \frac{d}{d\stepsize}q(0,0)
	 &= \begin{aligned}[t]
		&-\underbrace{\begin{pmatrix}
				\C_\Cost(x,D_{\hat{\prgrad}}x)
				\\
				\C_\Cost(D_{\hat{x}}x, D_{\hat{\prgrad}}x)
		  \end{pmatrix}^T 
	 }_{\overset{\eqref{eq: taylor cov - (Dv x, x)},\eqref{eq: taylor cov - (Dv x, Dw x)}}=0}
		  \Sigma^{-1}
		  \begin{pmatrix}
				\magenta{\bar{\Cost}(x)}
				\\
				\teal{D_{\hat{x}}\bar{\Cost}(x)}
		  \end{pmatrix}
		  \\
	 &\qquad- \underbrace{\frac{
		  \C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)
	 }{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)}}_{=1}
	 \teal{\bigl\|\prgrad\bigr\|}
	\end{aligned}
\end{align*}
Similarly we get for the second order derivatives
\begin{align*}
	 \frac{d^2}{(dh)^2}q(0,0)
	 &= \begin{aligned}[t]
		  &\begin{pmatrix}
				\C_\Cost(x,D_{\hat{x}}^2x)
				\\
				\blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}^2x)}
		  \end{pmatrix}^T 
		  \!\Sigma^{-1}\!
		  \begin{pmatrix}
				\magenta{\bar{\Cost}(x)}
				\\
				\teal{D_{\hat{x}}\bar{\Cost}(x)}
		  \end{pmatrix}
		  \\
		  &\qquad+ \underbrace{\frac{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{x}}^2x)}{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)}}_{
				\overset{\eqref{eq: taylor cov - (Dv x, Dw1 Dw2 x)}}= 0
		  }
		  \teal{\bigl\|\prgrad\bigr\|}
		  \\
		  &\qquad+ \mu''\bigl(\tfrac{\|x\|^2}2\bigr)\|x\|^2 + \mu'\bigl(\tfrac{\|x\|^2}2\bigr)
	 \end{aligned}
	 \\
	 \frac{d^2}{(d\stepsize)^2}q(0,0)
	 &= \begin{aligned}[t]
		  &\begin{pmatrix}
				\C_\Cost(x,D_{\hat{\prgrad}}^2x)
				\\
				\blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{\prgrad}}^2x)}
		  \end{pmatrix}^T 
		  \Sigma^{-1}
		  \begin{pmatrix}
				\magenta{\bar{\Cost}(x)}
				\\
				\teal{D_{\hat{x}}\bar{\Cost}(x)}
		  \end{pmatrix}
		  \\
		  &\qquad+ \underbrace{\frac{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}^2x)}{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)}}_{
				\overset{\eqref{eq: taylor cov - (Dv x, Dw1 Dw2 x)}}= 0
		  }
		  \teal{\bigl\|\prgrad\bigr\|}
		  + \mu'\bigl(\tfrac{\|x\|^2}2\bigr)
	 \end{aligned}
	 \\
	 \frac{d^2}{dh d\stepsize}q(0,0)
	 &= 
	 \begin{aligned}[t]
	 &\underbrace{
		  \begin{pmatrix}
				\C_\Cost(x, D_{\hat{x}}D_{\hat{\prgrad}}x)
				\\
				\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}D_{\hat{\prgrad}} x)
		  \end{pmatrix}^T
	 }_{
		  \overset{\eqref{eq: taylor cov - (Dv1 Dv2 x, x)},\eqref{eq: taylor cov - (Dv x, Dw1 Dw2 x)}}=0
	 }
	 \!\!\Sigma^{-1}\!
	 \begin{pmatrix}
		  \magenta{\bar{\Cost}(x)}
		  \\
		  \teal{D_{\hat{x}}\bar{\Cost}(x)}
	 \end{pmatrix}
	 \\
	 &+ \frac{\blue{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{x}}D_{\hat{\prgrad}}x)}}{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)}
	 \teal{\bigl\|\prgrad\bigr\|}.
	\end{aligned}
\end{align*}
In the affine isotropic case \(\Sigma\) is a diagonal matrix by
Lemma~\ref{lem: taylor covariance}, \eqref{eq: taylor cov - (Dv x, x)}
\begin{align*}
	 \Sigma &:= \Cov\Bigl(
		  \begin{pmatrix}
				\Cost(x)
				\\
				D_{\hat{x}}\Cost(x)
		  \end{pmatrix}
	 \Bigr)
	 \\
	 &= \begin{pmatrix}
		  \C_\Cost(x,x) & \blue{\C_\Cost(D_{\hat{x}}x ,x)}
		  \\
		  \blue{\C_\Cost(D_{\hat{x}}x ,x)} & \C_\Cost(D_{\hat{x}}x ,D_{\hat{x}} x)
	 \end{pmatrix}.
\end{align*}
Similarly all other terms marked in \blue{blue are zero} by \eqref{eq: taylor cov -
(Dv x, Dw1 Dw2 x)}. The claim follows by applying \eqref{eq: taylor cov - (Dv
x, Dw x)} and \eqref{eq: taylor cov - (Dv1 Dv2 x, x)} to the remaining
terms.

\subsection{Proof of Corollary~\ref{cor: a-rfd in the affine isotropic case}}

We get from Proposition~\ref{prop: tayloring the conditional expectation}
\begin{align*}
	 \begin{pmatrix}
		  \tilde{h}\\ \tilde{\stepsize}
	 \end{pmatrix} 
	 &= - [\nabla^2q(0,0)]^{-1}\nabla q(0,0)
	 \\
	 &= \frac{\ikernel(0)}{\ikernel'(0)\magenta{\bar{\Cost}(x)}}
	 \begin{pmatrix}
		  D_{\hat{x}}\Cost(x)\\
		  \|\prgrad\|
	 \end{pmatrix},
\end{align*}
such that
\begin{align*}
	 \tilde{d} &= \tilde{h}\hat{x} + \tilde{\stepsize}\hat{\prgrad}
	 \\
	 &= \frac{\ikernel(0)}{\ikernel'(0)\magenta{\bar{\Cost}(x)}}
	 \Bigl(
		  D_{\hat{x}}\Cost(x) \hat{x}
		  +  \|\prgrad\|\hat{\prgrad}
	 \Bigr)
	 \\
	 &= \frac{\ikernel(0)}{\ikernel'(0)\magenta{\bar{\Cost}(x)}} \nabla\Cost(x).
	 \qedhere
\end{align*}

\subsection{Asymptotic Step Sizes in the Linear Isotorpic Case}


\begin{prop}[Asymptoticially approximately optimal step in the non-stationary isotropic case]
	\label{prop: asymptotic approx optimal step}
    For \(\|\nabla\Cost(x)\|\to 0\), we have
    \[
        \begin{pmatrix}
            \tilde{h}
            \\
            \tilde{\stepsize}
        \end{pmatrix}
        \sim \begin{pmatrix}
                a & 0
                \\
                0 & b
            \end{pmatrix}^{-1}
        \begin{pmatrix}
            D_{\hat{x}}\Cost(x)
            \\
            \|\proj{x^\perp}\nabla\Cost(x)\|
        \end{pmatrix}
    \]
    with
    \begin{align*}
        b
        &= \begin{aligned}[t]
			&\tfrac{
				\C_\Cost(x, D_{\hat{\prgrad}}^2 x) \C_\Cost(D_{\hat{x}}x, D_{\hat{x}}x)
				- \blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{\prgrad}}^2x)\C_\Cost(D_{\hat{x}}x, x)}
			}{
				\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}x)\C_\Cost(x,x) - \blue{\C_\Cost(D_{\hat{x}}x, x)^2}
			}\magenta{\bar{\Cost}(x)}
			\\
			&+ \mu'\bigl(\tfrac{\|x\|^2}2\bigr)
		\end{aligned}
        \\
        a 
        &=\begin{aligned}[t]
            & \tfrac{
                \C_\Cost(x, D_{\hat{x}}^2 x) \C_\Cost(D_{\hat{x}}x, D_{\hat{x}}x)
                - \blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}^2x)\C_\Cost(D_{\hat{x}}x, x)}
            }{
                \C_\Cost(D_{\hat{x}}x, D_{\hat{x}}x)\C_\Cost(x,x) - \blue{\C_\Cost(D_{\hat{x}}x, x)^2}
            }\magenta{\bar{\Cost}(x)}
            \\
            &+ \mu''\bigl(\tfrac{\|x\|^2}2\bigr)\|x\|^2 + \mu'\bigl(\tfrac{\|x\|^2}2\bigr).
        \end{aligned}
    \end{align*}
\end{prop}
\begin{proof}
	Based on Lemma~\ref{lem: first taylor approx is asymptotically equal} our
	strategy will be to find the First Taylor approximation of \(\tilde{h}\) and
	\(\tilde{\stepsize}\)
	in \(\|\nabla\Cost(x)\|\). For this let
	\begin{align*}
			\epsilon &:= \|\nabla\Cost(x)\|
			\\
			\Theta_x &:= \frac{D_{\hat{x}} \Cost(x)}{\|\nabla\Cost(x)\|}  &&\in [-1,1]
			\\
			\Theta_\perp &:= \frac{\|\prgrad\|}{\|\nabla\Cost(x)\|} = \frac{\|\proj{x^\perp} \nabla\Cost(x)\|}{\|\nabla\Cost(x)\|}
			&& \in [0,1]
	\end{align*}
	such that \(\Theta_x^2 + \Theta_\perp^2= 1\). Then
	\[
			\nabla q(0,0) = - \epsilon \begin{pmatrix}
				\Theta_x \\ \Theta_\perp
			\end{pmatrix},
	\]
	and
	\begin{align*}
			H(\epsilon)
			&:=\nabla^2q(0,0)
			\\
			&= \begin{pmatrix}
				a & \epsilon\frac{
					\blue{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{x}}D_{\hat{\prgrad}}x)}
				}{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)}
				\Theta_\perp
				\\
				\epsilon\frac{
					\blue{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{x}}D_{\hat{\prgrad}}x)}
				}{\C_\Cost(D_{\hat{\prgrad}}x, D_{\hat{\prgrad}}x)}
				\Theta_\perp
				& b
			\end{pmatrix},
	\end{align*}
			
	where
	\begin{align*}
			a(\epsilon) &= \begin{aligned}[t]
				&\begin{pmatrix}
				\C_\Cost(x,D_{\hat{x}}^2x)
				\\
				\blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}^2x)}
			\end{pmatrix}^T 
			\! \Sigma^{-1}
			\begin{pmatrix}
				\magenta{\bar{\Cost}(x)}
				\\
				\teal{\epsilon \Theta_x}
			\end{pmatrix}
			\\
			&+ \mu''\bigl(\tfrac{\|x\|^2}2\bigr)\|x\|^2 + \mu'\bigl(\tfrac{\|x\|^2}2\bigr)
		\end{aligned}
			\\
			b(\epsilon) &= \begin{pmatrix}
				\C_\Cost(x,D_{\hat{\prgrad}}^2x)
				\\
				\blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{\prgrad}}^2x)}
			\end{pmatrix}^T 
			\! \Sigma^{-1}
			\begin{pmatrix}
				\magenta{\bar{\Cost}(x)}
				\\
				\teal{\epsilon \Theta_x}
			\end{pmatrix}
			+ \mu'\bigl(\tfrac{\|x\|^2}2\bigr).
	\end{align*}
	Therefore the function we need the first Taylor approximation of is
	\[
			f(\epsilon):=\begin{pmatrix}
				\tilde{h}\\ \tilde{\stepsize}
			\end{pmatrix}(\epsilon)
			= \epsilon H(\epsilon)^{-1}\begin{pmatrix}
				\Theta_x \\ \Theta_\perp
			\end{pmatrix}
	\]
	It is easy to see, that \(f(0) = 0\). Its derivative is given by
	\[
			H(\epsilon)^{-1}
			\begin{pmatrix}
				\Theta_x \\ \Theta_\perp
			\end{pmatrix}
			- \epsilon \Bigl[H(\epsilon)^{-1} \Bigl(\frac{dH(\epsilon)}{d\epsilon}\Bigr) H(\epsilon)^{-1}\Bigr]
			\begin{pmatrix}
				\Theta_x \\ \Theta_\perp
			\end{pmatrix}
	\]
	and thus
	\[
			f'(0) = H(0)^{-1}
			\begin{pmatrix}
				\Theta_x \\ \Theta_\perp
			\end{pmatrix}.
	\]
	Therefore
	\[
			g(\epsilon) = f(0) + f'(0)\epsilon = H(0)^{-1}\begin{pmatrix}
				D_{\hat{x}}\Cost(x)\\
				\|\proj{x^\perp}\nabla\Cost(x)\|
			\end{pmatrix}
	\]
	does the job.
	Here
	\[
			H(0)
			= \begin{pmatrix}
				a(0) & 0
				\\
				0 & b(0)
			\end{pmatrix},
	\]
	with
	\begin{align*}
		b(0) &= \begin{pmatrix}
			\C_\Cost(x,D_{\hat{\prgrad}}^2x)
			\\
			\blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{\prgrad}}^2x)}
		\end{pmatrix}^T 
		\! \Sigma^{-1}
		\begin{pmatrix}
			\magenta{\bar{\Cost}(x)}
			\\
			0
		\end{pmatrix}
		+ \mu'\bigl(\tfrac{\|x\|^2}2\bigr)
		\\
		&= \begin{aligned}[t]
		&\tfrac{
			\C_\Cost(x, D_{\hat{\prgrad}}^2 x) \C_\Cost(D_{\hat{x}}x, D_{\hat{x}}x)
			- \blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{\prgrad}}^2x)\C_\Cost(D_{\hat{x}}x, x)}
		}{
			\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}x)\C_\Cost(x,x) - \blue{\C_\Cost(D_{\hat{x}}x, x)^2}
		}\magenta{\bar{\Cost}(x)}
		\\
		&\qquad+ \mu'\bigl(\tfrac{\|x\|^2}2\bigr)
		\end{aligned}
		\\
		a(0) &= \begin{aligned}[t]
		&\begin{pmatrix}
			\C_\Cost(x,D_{\hat{x}}^2x)
			\\
			\blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}^2x)}
		\end{pmatrix}^T 
		\! \Sigma^{-1}
		\begin{pmatrix}
			\magenta{\bar{\Cost}(x)}
			\\
			0
		\end{pmatrix}
		\\
		&\qquad+ \mu''\bigl(\tfrac{\|x\|^2}2\bigr)\|x\|^2 + \mu'\bigl(\tfrac{\|x\|^2}2\bigr)
	\end{aligned}
		\\
		&=\begin{aligned}[t]
			& \tfrac{
				\C_\Cost(x, D_{\hat{x}}^2 x) \C_\Cost(D_{\hat{x}}x, D_{\hat{x}}x)
				- \blue{\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}^2x)\C_\Cost(D_{\hat{x}}x, x)}
			}{
				\C_\Cost(D_{\hat{x}}x, D_{\hat{x}}x)\C_\Cost(x,x) - \blue{\C_\Cost(D_{\hat{x}}x, x)^2}
			}\magenta{\bar{\Cost}(x)}
			\\
			&\qquad+ \mu''\bigl(\tfrac{\|x\|^2}2\bigr)\|x\|^2 + \mu'\bigl(\tfrac{\|x\|^2}2\bigr)
		\end{aligned}
	\end{align*}
	This finishes the proof.
\end{proof}

==> sections/extensions/linear_isotropy/quadratic_expectation.tex <==
\section{Quadratic expectation}\label{sec: non-constant expectation}

In this section we want to discuss the constant expectation assumption. In
principle, any expectation function \(m_\Cost\) is possible. Separating
\(\Cost\) into mean and centered random function \(\bar{\Cost}=\Cost-m_\Cost\),
allows us to rewrite the minimization problem of \ref{rfd} into
\[
	\min_y \E[\Cost(y)\mid \Cost(x), \nabla\Cost(x)]
	= \min_y m_\Cost(y) + \E[\bar{\Cost}(y) \mid \bar{\Cost}(x), \nabla\bar{\Cost}(x)].
\]
In this paper we essentially discuss minimization of the second summand. The 
mean can act as a regularizer.
In a linear model for example, the expectation turns out to be quadratic
(Section~\ref{sec: linear toy model}). This represents \(L^2\)-regularization, which
adds quadratic regularization to \(\Cost\), i.e.
\[
	f(\param) = \Cost(\param) + \rho \|\param\|^2 \quad\text{and thus}\quad
	\nabla f(\param) = \nabla \Cost(\param) + 2\rho\param.
\]
While a heuristic motivation of the \(L^2\)-regularization result
in the hyperparameter \(\rho\) without interpretation, a quadratic expectation
function is very interpretable.

If the expectation of \(\Cost\) is estimated in the model selection process,
Theorem~\ref{thm: regularized rfd} explains how \ref{rfd} then selects the
correct \(L^2\)-regularization parameter \(\rho\) automatically and therefore
provides a theoretical foundation for this heuristic. In this theorem
\(g(\stepsize)\) takes the place of \(\nabla f\).

\begin{theorem}[Regularized RFD]\label{thm: regularized rfd}
	For an \textbf{isotropic} random function \(\Cost\) with expectation
	\[
		\E[\Cost(\param)] = \sigma^2\|\param\|^2 + \mu,
	\]
	the regularized gradient (a convex combination of \(\nabla\Cost(\param)\) and
	the expected gradient)
	\[
		g(\stepsize) := 
		\tfrac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\Cost(\param)
		+\bigl(1- \tfrac{\sqC'(\stepsize^2)}{\sqC'(0)}\bigr)
		\underbrace{\grad \E[\Cost(\param)]}_{=2\sigma^2\param}
	\]
	is the result of \ref{rfd} 
	\begin{equation}\label{eq: reg rfd decent direction}
		\step(\hat{\stepsize}) 
		= -\tfrac{\hat{\stepsize}}{\|g(\hat{\stepsize})\|}  g(\hat{\stepsize})
		= \argmin_\step \E[\Cost(\param + \step)\mid \Cost(\param), \grad\Cost(\param)]
	\end{equation}
	with optimal step size
	\[
		\hat{\stepsize} = \argmin_\stepsize 
		\sigma^2 \stepsize^2
		+ \tfrac{\sqC(\stepsize^2)}{\sqC(0)}(\Cost(\param) - m_\Cost(\param))
		-  \stepsize \|g(\stepsize)\|.
	\]
\end{theorem}
\begin{remark}
Note that both \(\nabla\Cost\) and \(\nabla m_\Cost\) are scaled in \(g(\stepsize)\).
So \(g(\stepsize)\) can only be equal to \(\nabla f\) up to a constant. But this
constant is removed in \eqref{eq: reg rfd decent direction} due to
normalization.
\end{remark}
\begin{remark}
An anisotropic mean (in the sense of Remark~\ref{rem: anisotropy}) would
similarly result in Tikhonov regularization.
\end{remark}

A very salient feature of the quadratic mean is its unboundedness towards
infinity. Neuronal networks with bounded activation functions and bounded
data result in a bounded loss, constant expectation is therefore a more
plausible assumption in this case.




==> sections/extensions/linear_isotropy/random_regression.tex <==
\section{Random Regression}\label{sec: random regression}

In this section we explain how the linear regression problems
\citep[e.g.][]{paquetteHaltingTimePredictable2022} with a random true linear
model can be viewed as a special case of a more general random function
assumption and how Gaussian linear models essentially induce a Gaussian random
function as the loss.

\begin{definition}[Random Regression]
    \label{def: random regression}
    Let \(\rf\) be a random function, \(X\) a random input inducing a label
    \[
        Y = \rf(X) + \noise
    \]
    with noise \(\noise\), where \(\rf, X\) and \(\noise\) are independent.
    We define the random cost function to be the mean squared error
    \[
        \Cost(\param) = \E\bigl[ \tfrac12\| Y - f_\param(X)\|^2 \mid \rf\bigr]
    \]
    using a parametrized model \(f_\param(x) = f(\param,x)\) with parameter
    \(\param\in\real^\dims\). The stochastic loss functions
    \[
        \loss_i(\param) = \tfrac12\|Y_i - f_\param(X_i)\|^2,
    \]
    generated by iid copies \((X_i, \noise_i)\) of \((X,\noise)\) but the same \(\rf\),
    are also a family of identically distributed random functions.
\end{definition}

For the mean and covariance function of \(\rf\) we use the notation
\[
    \mu_{\rf}(x) := \E[\rf(x)], \quad \C_{\rf}(x,y):= \Cov(\rf(x),\rf(y)).
\]
In the case of Gaussian random functions these fully determine the distribution
of \(\rf\).

\begin{example}[Random Linear Regression]
    \label{ex: random linear regression I}
    A (Gaussian) random signal \(\signal\in \real^\dims\) induces a
    (Gaussian) random function
    \(
        \rf(x) = \langle \signal, x\rangle.
    \)
    Using a linear model \(f_\param(x) = \langle \param, x\rangle\) the
    empirical loss for a data size of \(n\) can be written as
    \[
        \Cost_n(\param)
        = \frac1{n} \sum_{i=1}^n \loss_i(\param)
        = \tfrac1{2n} \|\mathbf{Y} - \mathbf{X}\param\|^2,
    \]
    with data \(\mathbf{X} = (X_1,\dots, X_n)^T\in \real^{\dims\times n}\) and
    labels \(\mathbf{Y}=(Y_1,\dots,Y_n)^T\in \real^n\). This is the linear regression
    considered by \citet{paquetteHaltingTimePredictable2022}. By the law of large numbers
    \(\Cost_n(\param)\to\Cost(\param)\). Assuming centered
    and whitened input (i.e. \(\E[XX^T] = \identity\)), it is straightforward to calculate
    \[
        \Cost(\param)
        = \tfrac12\|\param - \signal\|^2 + \tfrac12\E\noise^2,
        \qquad \nabla\Cost(\param) = \param-\signal.
    \]
    Gradient descent with step size one would therefore converge in one
    step, i.e. the problem is trivial. 
    \citet{paquetteHaltingTimePredictable2022} consider a more challenging
    setting, where the number of parameters is proportional to the amount of
    data, i.e. \(\dims/n\to r \in (0,\infty)\) as \(n\to\infty\).
\end{example}

In non-linear random regression \(\Cost\) is a much more complex object by itself. In
particular, it is not necessarily convex like in random linear regression. So we
focus on \(\Cost\) for now, i.e. the setting with an infinite source of data. 
Interestingly, the loss \(\Cost\) is essentially Gaussian, if we
start from a Gaussian random function \(\rf\) (see~Theorem~\ref{thm: general
regression decomposition}).

\begin{theorem}[General Regression Decomposition]
    \label{thm: general regression decomposition}
    \(\Cost\) as defined in Definition~\ref{def: random regression} can be
    decomposed into
    \[
        \Cost(\param)
        = \underbrace{\mu_\Cost(\param)}_{\text{deterministic}}
        + \underbrace{Z}_{\text{random shift}}
        + \underbrace{\hat{\Cost}(\param)}_{\text{random function}}.
    \]
    The expectation
    \[
        \mu_\Cost(\param)
        = \tfrac12\E\|f_\param(X) -\mu_{\rf}(X)\|^2 + \E\Bigl[\tfrac{\trace\C_{\rf}(X,X) + \|\noise\|^2}2\Bigr]
    \]
    is constant if \(\rf\) has constant expectation \(\mu_{\rf}\equiv\mu\in\real\), and the
    output of \(f_\param\) is batch normalized 
    \citep{ioffeBatchNormalizationAccelerating2015} with infinite batch size.
    \(Z\) is a centered random
    variable and \(\hat{\Cost}\) a centered random function with covariance 
    \begin{align*}
        \C_{\hat{\Cost}}(\param_1, \param_2)
        &= \begin{aligned}[t]
            \iint &\bigl(f_{\param_1}(x)-\mu_{\rf}(x)\bigr)^T 
            \C_{\rf}(x,y)
            \\
            &\cdot \bigl(f_{\param_2}(y)-\mu_{\rf}(y)\bigr)
            \Pr_X(dx) \Pr_X(dy).
        \end{aligned}
    \end{align*}
    If \(\rf\) is Gaussian, then \(\hat{\Cost}\) is Gaussian.
\end{theorem}

\begin{remark}[Why \(Z\) does not matter]
    While \(Z\) changes the distribution of \(\Cost\) in principle, it has no bearing on
    minima or gradients. Furthermore, any estimation of the mean which relies
    on multiple evaluations of \(\Cost\) and ergodicity will capture and remove \(Z\)
    from the centered version of \(\Cost\). So if \(\rf\) is Gaussian, \(\Cost\) is
    essentially Gaussian.
\end{remark}

\begin{example}[Random Linear Regression]
    \label{ex: random linear regression II}
    Assuming whitened input, recall from Example~\ref{ex: random linear
    regression I} the loss induced by random linear regression is of the form
    \begin{align*}
        \Cost(\param)
        &= \tfrac12\|\param - \signal\|^2 + \tfrac12\E\noise^2,
        \\
        &= \underbrace{
            \tfrac{\|\param\|^2}2 + \E\Bigl[\tfrac{\|\signal\|^2 + \noise^2}2\Bigr]
        }_{=\mu_\Cost(\param)}
        + \underbrace{\tfrac{\|\signal\|^2 - \E\|\signal\|^2}2}_{=Z}
        \underbrace{- \langle\param, \signal\rangle}_{=\hat{\Cost}(\param)},
    \end{align*}
    where we assumed \(\signal\) is centered; otherwise
    replace all \(\param\) by \(\param-\E[\signal]\) and \(\signal\) by
    \(\signal-\E[\signal]\).
    Further assuming \(\E[\signal\signal^T] = \frac{\sigma^2}{\dims} \identity\) like 
    \citet{paquetteHaltingTimePredictable2022}, we get
    \[
        \C_{\hat{\Cost}}(x,y) = \C_{\rf}(x,y) = \tfrac{\sigma^2}{\dims}\langle x,y\rangle.
    \]
    This is an example for a non-stationary isotropic random function, which we will
    introduce in the next section.
\end{example}

==> sections/extensions/linear_isotropy/regularized_rfd.tex <==
\section{Regularized RFD}\label{sec: regularized rfd}

The previous section motivated
\[
	m_\Cost(\param) := \E[\Cost(\param)] = \sigma^2\|\param\|^2 + \mu.
\]
Turning this into an assumption without regard for its origin results in a form
of \(L_2\)-regularization of the RFD optimization problem. We assume
that
\[
	\bar{\Cost}=\Cost-m_\Cost
\]
is isotropic and get due to linearity of the \(\BLUE\)
\begin{equation*}
	\BLUE[\Cost(\param+\step)\mid \Cost(\param), \grad\Cost(\param)]
	= m_\Cost(\param+\step) + \frac{\sqC(\|\step\|^2)}{\sqC(0)}\bar{\Cost}(\param)
	+ \frac{\sqC'(\|\step\|^2)}{\sqC'(0)}\langle \step, \grad\bar{\Cost}(\param)\rangle
\end{equation*}
with
\begin{align*}
	\bar{\Cost}(\param)
	&= \Cost(\param) - (\sigma^2 \|\param\|^2 + \mu)\\
	\grad\bar{\Cost}(\param)
	&= \grad\Cost(\param) - 2\sigma^2 \param
\end{align*}
Since the direction of \(\step\) matters in more than one place now, the
minimization problem becomes more complicated. But we still want to do the
minimization over \(\step\) in two steps. First we fix some \(\stepsize=\|\step\|\)
and then we optimize over \(\stepsize\). To solve the restricted optimization problem
we define the Lagrangian function
\begin{equation*}
	L(\step, \lambda) := \BLUE[\Cost(\param+\step)\mid \Cost(\param),\grad\Cost(\param)]	
	+ \lambda(\|\step\|^2 - \stepsize^2)
\end{equation*}
Taking the derivative with respect to \(\step\) results in
\begin{align*}
	0\overset!=\grad_\step L(\step,\lambda)
	&= \grad m_\Cost(\param+\step)
	+ \frac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\bar{\Cost}(\param)
	+ 2\lambda\step
	\\
	&= 2\sigma^2(\param + \step)
	+ \frac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\bar{\Cost}(\param)
	+ 2\lambda\step
\end{align*}
This implies that
\begin{equation*}
	\step = 
	- \frac{
		\frac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\bar{\Cost}(\param)
		+ 2\sigma^2 \param
	}{2\sigma^2 + 2\lambda}.
\end{equation*}
Taking the derivative of the Lagrangian with respect to \(\lambda\) would
provide us with the constraint \(\|\step\|=\stepsize\) again. And since \(2\sigma^2
+ 2\lambda\) is a real number we can move out of the norm, we get
\begin{equation*}
	\frac\step\stepsize = \frac{\step}{\|\step\|}
	= - \frac{
		\frac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\bar{\Cost}(\param)
		+ 2\sigma^2 \param
	}{\left\|
		\frac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\bar{\Cost}(\param)
		+ 2\sigma^2 \param
	\right\|}.
\end{equation*}
Note that this is where a more complicated mean like \(m_\Cost(\param) =
\param^T \Sigma_X \param\) would fail, as we can not move \(\Sigma_X\) out of
the norm. Which is why it was important to rescale the bias in the linear model.
In conclusion we have
\begin{equation*}
	\step(\stepsize) = -\stepsize \frac{
		\frac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\bar{\Cost}(\param)
		+ 2\sigma^2 \param
	}{\left\|
		\frac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\bar{\Cost}(\param)
		+ 2\sigma^2 \param
	\right\|}.
\end{equation*}
I.e. we have
\begin{align*}
	\step(\stepsize) 
	&\sim \underbrace{\frac{\sqC'(\stepsize^2)}{\sqC'(0)}}_{\text{trust decay}}
	\overbrace{
		(\grad\Cost(\param) - \grad m_\Cost(\param))
	}^{\grad\bar{\Cost}(\param)}
	+ \underbrace{1}_{\text{no decay}}\grad m_\Cost(\param) \\
	&= \frac{\sqC'(\stepsize^2)}{\sqC'(0)} \grad\Cost(\param)
	+\left(1- \frac{\sqC'(\stepsize^2)}{\sqC'(0)}\right) \grad m_\Cost(\param).
\end{align*}
In other words: We start out moving in the direction of the gradient, \(\step(0)
\sim \grad\Cost(\param)\), but with increasing distance \(\stepsize=\|\step\|\) from
\(\param\), we trust the gradient less and less and increasingly move in the
direction of the gradient of the mean \(\grad m_\Cost\).

Recall that \(L_2\)-regularization of the loss implies
\[
	f(\param) := \Cost(\param) + \lambda\|\param\|^2
\]
and the gradient would then be
\[
	\grad f(\param) = \nabla\Cost(\param) + 2\lambda\param.
\]
So in some sense we are simply selecting a dynamic regularization \(\lambda\) with
\begin{equation*}
	\frac{\lambda}{1+\lambda} = 1 - \frac{\sqC'(\stepsize^2)}{\sqC'(0)},
\end{equation*}
where the regularization term increases with \(\stepsize\). Resubstituting the
direction \(\step(\stepsize)\) back into the \(\BLUE\) we get
\begin{align*}
	&\BLUE[\Cost(\param + \step(\stepsize))\mid \Cost(\param), \grad\Cost(\param)]
	\\
	&= \sigma^2\|\param + \step(\stepsize)\|^2 + \mu 
	+ \frac{\sqC(\stepsize^2)}{\sqC(0)}\bar{\Cost}(\param)
	+ \frac{\sqC'(\stepsize^2)}{\sqC'(0)} \langle \step(\stepsize), \grad\bar{\Cost}(\param)\rangle
	\\
	&= \mu + \sigma^2(\|\param\|^2 + 2\langle \param, \step(\stepsize)\rangle +\stepsize^2)
	+ \frac{\sqC(\stepsize^2)}{\sqC(0)}\bar{\Cost}(\param)
	+  \left\langle \step(\stepsize), \frac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\bar{\Cost}(\param)\right\rangle
	\\
	&= C + \sigma^2 \stepsize^2
	+ \frac{\sqC(\stepsize^2)}{\sqC(0)}\bar{\Cost}(\param)
	+  \underbrace{\left\langle
		\step(\stepsize),
		\frac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\bar{\Cost}(\param)
		+ 2\sigma^2\param
	\right\rangle}_{
		= -\stepsize \left\|
		\frac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\bar{\Cost}(\param)
		+ 2\sigma^2\param
		\right\|
	},
\end{align*}
where \(C\) is a constant independent of \(\stepsize\).
\begin{theorem}[Regularized RFI Descent]
	For an \textbf{isotropic} random function \(\Cost\) with mean
	\[
		\E[\Cost(\param)] = \sigma^2\|\param\|^2 + \mu,
	\]
	the regularized gradient (a convex combination of \(\nabla\Cost(\param)\) and
	the expected gradient)
	\[
		g(\stepsize) := 
		\frac{\sqC'(\stepsize^2)}{\sqC'(0)}\grad\Cost(\param)
		+\left(1- \frac{\sqC'(\stepsize^2)}{\sqC'(0)}\right)
		\underbrace{\grad \E[\Cost(\param)]}_{=2\sigma^2\param}
	\]
	is the maximum descent direction for the 1-step 1-order \(\BLUE\). I.e.
	\begin{equation*}
		\step(\hat{\stepsize}) 
		= -\hat{\stepsize} \frac{g(\hat{\stepsize})}{\|g(\hat{\stepsize})\|}
		= \argmin_\step \BLUE[\Cost(\param + \step)\mid \Cost(\param), \grad\Cost(\param)]
	\end{equation*}
	with
	\[
		\hat{\stepsize} = \argmin_\stepsize 
		\sigma_X^2 \stepsize^2
		+ \frac{\sqC(\stepsize^2)}{\sqC(0)}(\Cost(\param) - m_\Cost(\param))
		-  \stepsize \|g(\stepsize)\|.
	\]
\end{theorem}



==> sections/extensions/linear_isotropy/toy-models.tex <==
\section{Toy models}\label{sec: toy-models}

This section investigates the plausibility of the constant expectation
assumption.

\subsection{A linear model}

Let us assume that the real data labels are generated by
\[
	Y = \theta_1^T X + \epsilon \in \real
\]
with inputs
\[
	X = \theta_2 \Theta \in \real^\dims
\]
So the randomness is driven by output randomness \(\epsilon\) with \(\E[\epsilon]=0\) and variance
\(\sigma^2\) and input randomness \(\Theta\in\real^m\) with iid entries of unit variance.
We also use a linear model for regression
\begin{equation}\label{eq: linear regression}
	f(\param, x) = \param^T x,
\end{equation}
and use the mean squared cost function
\[
	\Cost(\param) = \E[(Y - \param^T X)^2 \mid \theta].
\]
We conditioned on the ``real parameters'' \(\theta\) here, so we should probably
talk about its prior distribution now. So first, we would like \(\theta_1\in \real^\dims\)
and \(\theta_2\in \real^{\dims \times m}\) to be independent (or at least \(\E[\theta_2\theta_2^T\mid
\theta_1]\) to be constant), second they should also be independent of \(\epsilon\)
and \(\Theta\). Finally let us assume \(\E[\theta_1]=0\).

\begin{prop}[Explicit loss in the linear model]
	For the linear probability model above, we get
	\[
		\Cost(\param)
		= (\theta_1 - \param)^T \theta_2 \theta_2^T (\theta_1 - \param)
		+ \sigma^2.
	\]
	And with \(\E[\theta_2\theta_2^T] =: \Sigma\), we can obtain
	\[
		\E[\Cost(\param)]
		= \param^T \Sigma \param 
		+ \underbrace{\E[\theta_1^T \Sigma \theta_1] + \sigma^2}_{=:\mu}
		= \|w\|_\Sigma^2 + \mu
	\]
\end{prop}
\begin{proof}
	First we calculate \(\Cost\)
	\begin{align*}
		\Cost(\param)
		&= \E[(Y - \param^T X)^2 \mid \theta]\\
		&= \E[( (\theta_1 - \param)^T X + \epsilon)^2 \mid \theta]\\
		&= \E[((\theta_1-\param)^T X)^2 \mid \theta]
		+ 2
			\E[((\theta_1-\param)^TX)\underbrace{\E[\epsilon\mid \theta, X]}_{=0}\mid \theta]
		+ \underbrace{\E[\epsilon^2]}_{=\sigma^2}\\
		&= \E[
			(\theta_1-\param)^T \theta_2 \Theta \Theta^T \theta_2^T (\theta_1-\param)
			\mid \theta
		]
		+ \sigma^2\\
		\overset{\E[\Theta\Theta^T]=\identity}&= 
		(\theta_1-\param)^T \theta_2\theta_2^T (\theta_1-\param)
		+ \sigma^2.
	\end{align*}
	Then we calculate its expectation
	\begin{align*}
		\E[\Cost(\param)]
		&= \E[(\theta_1-\param)^T \underbrace{
			\E[\theta_2\theta_2^T\mid \theta_1]
		}_{=\Sigma}
		(\theta_1-\param)] + \sigma^2\\
		&= \E[\theta_1^T \Sigma \theta_1]
		+ 2\param^T\Sigma\underbrace{\E[\theta_1]}_{=0}
		+ \param^T\Sigma\param + \sigma^2.\qedhere
	\end{align*}
\end{proof}

Notice how \(\theta_2\in \real^{\dims\times m}\) allows for a complex
input data distribution \(X\) by cranking up \(m\). If we draw all entries
of \(\theta_2\) iid Gaussian and assume \(m\ge\dims\),
\(\theta_2\theta_2^T\) is Wishart distributed. In particular we have
\(\E[\theta_2\theta_2^T] = m\identity\). In that case the mean is rotation
invariant, i.e.
\[
	\E[\Cost(\param)] = m\|\param\|^2 + \mu.
\]


\subsection{Labels as a random function}

We could also have defined the labels
\[
	Y = f(\theta_1, X) + \epsilon
\]
using the linear model \(f\), we used for regression in \eqref{eq: linear
regression}.  We now want to consider a more general model \(g(\theta_1,x)\) and
drop the measurement error \(\epsilon\), since it should be clear, that it will
only materialize in a constant increase of the expected loss. Notice how we can
always view
\[
	Z(x) := g(\theta_1, x)
\]
as a random function into which we plug the data \(X\). We continue to assume
\(X=\theta_2 \Theta\) with independency between \(\theta_1\), \(\theta_2\) and
\(\Theta\), And assume that \(Z\) centered. Then we have
\begin{equation*}
	\Cost(\param)
	= \E[\|f(\param, X) - Y\|^2 \mid \theta]
	= \E[\|f(\param, X) - Z(X)\|^2 \mid \theta].
\end{equation*}
It now makes sense to calculate a conditional mean first
\begin{align*}
	m_X(\param)&:= \E[\|\model{X}-Z(X)\|^2 \mid X]\\
	&= \|\model{X}\|^2 - 2\langle \model{X}, \underbrace{\E[Z(X)\mid X]}_{=0}\rangle
	+ \underbrace{\E[\|Z(X)\|^2\mid X]}_{=:\sigma_Z^2(X)}\\
	&= \|\model{X}\|^2 + \sigma_Z^2(X).
\end{align*}
Where we have used that \(\E[Z(x)]=0\) and the independence of \(Z\) and \(X\)
for \(\E[Z(X)\mid X]=0\). By the tower property of conditional expectation we
now get
\begin{equation*}
	\E[\Cost(\param)]
	= \E[m_X(\param)]
	= \E\|\model{X}\|^2 + \underbrace{\E[\sigma_Z^2(X)]}_{=:\mu \in\real}.
\end{equation*}

So in general up to a constant, we could try to calculate \(\E\|f(\param,
X)\|^2\) to get the expectation of the loss. A linear model \(f\) will lead
to a quadratic mean. A bounded model \(f\) has a much better chance to have
constant expectation on the other hand. But before we consider bounded models,
let us use this insight to calculate the expectation of a linear model with
bias.
\subsection{Linear regression with bias}

We consider \(\mathbf{\param} = (\param, \param_0)\) and \(X=\theta_2 \Theta\) with
\(\theta_2\in \real^{\dims\times m}\) for \(m\ge \dims\) and iid
\(\normal(0,1)\) entries for simplicity and define the regression to be
\begin{equation*}
	f(\mathbf{\param}, X) = X^T\param + \sqrt{m}\param_0 \in \real,
\end{equation*}
The normalization of the bias immediately makes sense once we calculate the
resulting mean
\begin{align*}
	\E\|f(\mathbf{\param}, X)\|^2
	&= \param^T \underbrace{\E[X X^T]}_{=\E[\theta_2 \mathrlap{\E[\Theta \Theta^T\mid\theta] \theta_2^T]}} \param
	+ 2\sqrt{m}\param_0\underbrace{\E[X^T]}_{=0}\param
	+ m\param_0^2\\
	&=(\param^T \E[\theta_2\theta_2^T]\param + m\param_0^2)\\
	&= m \|\mathbf{\param}\|^2,
\end{align*}
where we used the property \(\E[\theta_2\theta_2^T] = m \identity\) of
the Wishart matrix \(\theta_2\theta_2^T\).






==> sections/extensions/second_order_blue.tex <==
\section{Second order methods}

This section is a final addendum which was not discussed in the main work. Since
we were able to derive gradient descent from conditional expectation, it is
natural to ask, whether it might be possible to derive higher order methods,
like the Newton method from a conditional expectation too. While we were able
to recognize a Taylor-like component in the second order conditional expectation,
this approach has overall felt like a dead end, especially because second order
methods are not common in machine learning in the first place. But perhaps this
will be a useful starting point for future research.

\begin{lemma}
	If \(\Cost\) is a \textbf{centered, intrinsically stationary, twice
	differentiable} random function, with \textbf{rotation invariant} variogram
	\(\variogram\) of the form \(\variogram(\step)=\phi(\|\step\|^2)\), then
	\begin{equation*}
	\begin{aligned}
		&\BLUE[
			\underbrace{\Cost(\param+\step) - \Cost(\param)}_{=:\Cost_\param(\step)}
			\mid \grad\Cost(\param), \hessian\Cost(\param)
		]\\
		&=\begin{aligned}[t]
			&\underbrace{
				\frac{\phi'(\|\step\|^2)}{\phi'(0)}\langle \step, \grad\Cost(\param)\rangle
				- \frac{\phi''(\|\step\|^2)}{\phi''(0)}
				\frac12\langle \hessian\Cost(\param)\step, \step\rangle
			}_{\text{Taylor-like}}\\
			&+ \frac{\trace(\hessian \Cost(\param))}{\dims+2}\left[
				\frac{\phi'(0) - \phi'(\|\step\|^2)}{2\phi''(0)}
				+ \frac{\phi''(\|\step\|^2)}{2\phi''(0)}\|\diag(\step)\|^2
		\right].
		\end{aligned}
	\end{aligned}
	\end{equation*}
\end{lemma}

\begin{proof}
	We have
	\begin{equation*}
		\hat{\Cost}_\param(\step)
		= \langle b, \grad\Cost(\param)\rangle
		+ \underbrace{\sum_{ij} \partial_{ij}\Cost(\param) c_{ij}}_{
			=: \langle \hessian\Cost(\param), c\rangle}
	\end{equation*}
	where due to \(\partial_{ij}\Cost = \partial_{ji}\Cost\) only the sum \(c_{ij} + c_{ji}\) matters
	and we can assume without loss of generality \(c_{ij} = c_{ji}\). We want to
	minimize
	\begin{align*}
		g(b, c)
		&= \E[\|\Cost_\param(\step) - \hat{\Cost}_\param(\step)\|^2]\\
		&= \begin{aligned}[t]
			&\E[\Cost_\param(\step)^2]\\
			&- 2\langle b , \E[\Cost_\param(\step)\grad\Cost(\step)]\rangle
			+ \langle b, \E[\grad\Cost(\param) \grad\Cost(\param)^T]b\rangle \\
			& - \langle \E[\Cost_\param(\step)\hessian\Cost(\param)], c \rangle
			+ \E\left[\bigg(\sum_{i,j} \partial_{ij}\Cost(\param) c_{ij}\bigg)^2\right]
		\end{aligned}\\
		\overset{\text{Lem~\ref{lem: variogram and derivative}}}&= 2\variogram(\step)
		\begin{aligned}[t]
		&- 2\langle b, \grad\variogram(\step)\rangle
		+ \langle b, \hessian\variogram(0) b\rangle\\
		&- 2\langle \hessian\variogram(0) - \hessian\variogram(\step), c\rangle
		+ \sum_{l,k,i,j} \partial_{lkij} \variogram(0) c_{lk}c_{ij}
		\end{aligned}
	\end{align*}
	where we have used the fact that the first and second derivative are uncorrelated.
	Since \(b\) and \(c\) are in this sense independent form each other, optimizing
	\(g\) over \(b\) results in the same factor as in Lemma~\ref{lem: blue
	centered, intrinsically stationary}. So we just need to consider the optimization
	over \(c\). The first order condition is
	\begin{equation*}
		0 \overset!= \frac12\frac{dg}{dc_{ij}}
		= - \partial_{ij}[\variogram(0) - \variogram(\step)]
		+ \sum_{l,k} \partial_{lkij}\variogram(0) c_{lk}
	\end{equation*}
	As we are in the rotational invariant case \(\variogram(\step) = \phi(\|\step\|^2)\)
	we have (Lemma~\ref{lem: derivatives of rotation invariant variograms})
	\begin{align*}
		\partial_{ij}\variogram(\step)
		&= 4\phi''(\|\step\|^2)\step_i\step_j + 2\phi'(\|\step\|^2)\delta_{ij}\\
		\partial_{lkij}\variogram(0)
		&=4\phi''(0)[\delta_{ki}\delta_{jl} + \delta_{kj}\delta_{il} + \delta_{ij}\delta_{kl}].
	\end{align*}
	Which simplifies the first order condition to
	\begin{align*}
		0 \overset!= \frac12\frac{dg}{dc_{ij}}
		&= \begin{aligned}[t]
			&4\phi''(\|\step\|^2)\step_i\step_j + 2\phi'(\|\step\|^2)\delta_{ij}
			- 2\phi'(0)\delta_{ij}\\
			&+ 4\phi''(0)\sum_{l,k}[\delta_{ki}\delta_{jl} + \delta_{kj}\delta_{il} + \delta_{ij}\delta_{kl}]c_{lk}
		\end{aligned}\\
		&= \begin{aligned}[t]
			&4\phi''(\|\step\|^2)\step_i\step_j + 2[\phi'(\|\step\|^2)-\phi'(0)]\delta_{ij}\\
			&+ 4\phi''(0)\left[c_{ji} + c_{ij} + \delta_{ij}\diag(c)\right]
		\end{aligned}
	\end{align*}
	Taking another derivative in \(c\) results in a multiple of \(4\phi''(0)\)
	which is greater zero. Therefore the first order condition describes a
	minimum. Recall that we have have assumed \(c_{ij} = c_{ji}\) without
	loss of generality. So for \(i\neq j\) we have
	\begin{equation*}
		0\overset!= \phi''(\|\step\|^2)\step_i\step_j + 2\phi''(0)c_{ij}
	\end{equation*}
	which implies
	\begin{equation*}
		c_{ij} = - \frac{\phi''(\|\step\|^2)}{2\phi''(0)}\step_i\step_j.
	\end{equation*}
	On the diagonal on the other hand
	\begin{equation*}
		0\overset!= \phi''(\|\step\|^2)\step_i\step_i + \tfrac12[\phi'(\|\step\|^2)-\phi'(0)]
		+ \phi''(0)[2c_{ii} + \diag(c)]
	\end{equation*}
	which implies
	\begin{equation*}
		c_{ii} = -\left[
			\frac{\phi''(\|\step\|^2)}{2\phi''(0)}\step_i\step_i
			+ \frac{\tfrac12[\phi'(\|\step\|^2)-\phi'(0)]}{2\phi''(0)}
			+ \frac{\diag(c)}{2}
		\right].
	\end{equation*}
	Of course this is still recursive due to the diagonal. But	
	\begin{equation*}
		\diag(c)
		= - \frac{\phi''(\|\step\|^2)}{2\phi''(0)}\sum_{i}\step_i^2
		- \frac{\dims}2\frac{\phi'(\|\step\|^2) - \phi'(0)}{2\phi''(0)}
		- \frac{\dims}2 \diag(c)
	\end{equation*}
	implies
	\begin{equation*}
		\diag(c)
		= - \frac{
			\frac{\phi''(\|\step\|^2)}{2\phi''(0)}\sum_{i}\step_i^2
			+ \frac{\dims}2\frac{\phi'(\|\step\|^2) - \phi'(0)}{2\phi''(0)}
		}{1+\frac{\dims}2}.
	\end{equation*}
	So we finally end up with
	\begin{equation*}
		c_{ij} =
		\begin{aligned}[t]
			&- \frac{\phi''(\|\step\|^2)}{2\phi''(0)}\step_i\step_j\\
			&- \delta_{ij}\underbrace{\left[
			\frac{\tfrac12[\phi'(\|\step\|^2)-\phi'(0)]}{2\phi''(0)}
			- \frac{
				\frac{\phi''(\|\step\|^2)}{2\phi''(0)}\sum_{i}\step_i^2
				+ \frac{\dims}2\frac{\phi'(\|\step\|^2) - \phi'(0)}{2\phi''(0)}
			}{2(1+\frac{\dims}2)}
			\right]}_{=:I}.
		\end{aligned}
	\end{equation*}
	where we can further simplify \(I\) to
	\begin{align*}
		I
		&= 
		\left(1- \frac{\dims}{2+\dims}\right)\frac{\tfrac12[\phi'(\|\step\|^2)-\phi'(0)]}{2\phi''(0)}
		- \frac{
			\frac{\phi''(\|\step\|^2)}{2\phi''(0)}\|\diag(\step)\|^2
		}{2+\dims}\\
		&= \frac1{2+\dims}\left[
		\frac{\phi'(\|\step\|^2)-\phi'(0)}{2\phi''(0)}
		-
			\frac{\phi''(\|\step\|^2)}{2\phi''(0)}\|\diag(\step)\|^2
		\right].
	\end{align*}
	So the BLUE is of the form
	\begin{equation*}
		\BLUE[\Cost_\param(\step)\mid \grad\Cost(\param), \hessian\Cost(\param)]
		= \frac{\phi'(\|\step\|^2)}{\phi'(0)}\langle \step, \grad\Cost(\param)\rangle
		+ \sum_{ij}\partial_{ij}\Cost(\param)c_{ij}
	\end{equation*}
	with
	\begin{equation*}
		c_{ij} =
			- \frac{\phi''(\|\step\|^2)}{2\phi''(0)}\step_i\step_j
			+ \frac{\delta_{ij}}{\dims+2}\left[
				\frac{\phi'(0) - \phi'(\|\step\|^2)}{2\phi''(0)}
				+ \frac{\phi''(\|\step\|^2)}{2\phi''(0)}\|\diag(\step)\|^2
			\right].
	\end{equation*}
	Plugging these \(c_{ij}\) into the BLUE yields the claim.
\end{proof}

